Towards General Error Diagnosis via Behavioral Testing in Machine Translation

Behavioral testing offers a crucial means of diagnosing linguistic errors and assessing capabilities of NLP models. However, applying behavioral testing to machine translation (MT) systems is challenging as it generally requires human efforts to craft references for evaluating the translation quality of such systems on newly generated test cases. Existing works in behavioral testing of MT systems circumvent this by evaluating translation quality without references, but this restricts diagnosis to specific types of errors, such as incorrect translation of single numeric or currency words. In order to diagnose general errors, this paper proposes a new Bilingual Translation Pair Generation based Behavior Testing (BTPGBT) framework for conducting behavioral testing of MT systems. The core idea of BTPGBT is to employ a novel bilingual translation pair generation (BTPG) approach that automates the construction of high-quality test cases and their pseudoreferences. Experimental results on various MT systems demonstrate that BTPGBT could provide comprehensive and accurate behavioral testing results for general error diagnosis, which further leads to several insightful findings. Our code and data are available at https: //github.com/wujunjie1998/BTPGBT.

==> sections/chatgpt_infilling.tex <==
\section{Constrained Bilingual Translation Pair Generation}
\label{method}

\subsection{Problem Setup}
Consider a translation pair $(\boldsymbol{x}, \boldsymbol{y})$ %source sentence $\boldsymbol{x}$ and its reference translation $\boldsymbol{y}$, 
%an evaluation set for NMT systems  
where $\boldsymbol{x}$ and $\boldsymbol{y}$ refer to the source sentence and reference translation, respectively. The goal of constrained bilingual translation pair generation is to craft a new translation pair $\lbrace(\boldsymbol{x'}, \boldsymbol{y’})\rbrace$ through paraphrasing $(\boldsymbol{x}, \boldsymbol{y})$, while making sure that: 1): $\boldsymbol{x'}$ and $\boldsymbol{y'}$ are still fluent sentences; 2): $\boldsymbol{y'}$ is the reference translation of $\boldsymbol{x'}$.  
%By doing so, we could significantly increase the size of existing evaluation sets of NMT systems without much human effort to obtain more comprehensive evaluation results.

\subsection{Our Approach}
%A straightforward way to achieve the above goal is first paraphrase $\boldsymbol{x}$ to craft $\boldsymbol{x'}$, then use an NMT system to translate $\boldsymbol{x'}$ and obtain $\boldsymbol{y'}$. 
The overall process of our approach is shown in Figure X. 

\paragraph{Determining the Modification Positions}
%As mentioned in \sref{introduction}, bilingual translation pair generation is challenging since a small modification on the source sentence might largely shift its semantic meaning and leads to great efforts on crafting its reference translation. To tackle this issue, we constrain that only segments in the source sentence that have explicit alignments in the reference translation can be modified,  the rephrasing of . 

Given the source sentence $\boldsymbol{x}=(x_{1},\cdots,x_{n})$ and its reference $\boldsymbol{y}=(y_{1},\cdots,y_{m})$, the first step is to obtain segment-level alignments between $\boldsymbol{x}$ and $\boldsymbol{y}$, %for the mask-then-infill process, since 
where segments consist of words and phrases. The idea of targeting segment-level alignments rather than word-level alignments is to craft more diverse translation pairs during the mask-then-infill process. To find out all phrases in both $\boldsymbol{x}$ and $\boldsymbol{y}$, we use Stanza~\footnote{https://stanfordnlp.github.io/stanza/} to parse their corresponding syntax trees and pick phrases from their leaf nodes. 
%in varied lengths. 
Next, 
%a translation pair $(\boldsymbol{x}, \boldsymbol{y})$, 
we apply an open-source tool \jw{what is the tool?} to obtain a word-to-word alignment between $\boldsymbol{x}$ and $\boldsymbol{y}$ and use it to extract segment-level alignments. %between $\boldsymbol{x}$ and $\boldsymbol{y}$. 
%As mentioned in \sref{introduction}, generating a high-quality reference translation for a source sentence usually needs much manual efforts and thus limits the scale of bilingual translation pair generation. To tackle this issue, 
%In this work, we define segment as a word or several continuous words 
Three types of segment-level alignments will be extracted:
\begin{enumerate}
    \item a word in $\boldsymbol{x}$ that only aligns with a word or a phrase in $\boldsymbol{y}$.
    \item a word in $\boldsymbol{y}$ that only aligns with a word or a phrase in $\boldsymbol{x}$.
    \item a phrase in $\boldsymbol{x}$ that only aligns with a phrase in $\boldsymbol{y}$.
\end{enumerate}
\iffalse
For the first two types of alignments, we could simply pick them from the word-to-word alignment. As for the third type, 
%For each word $x_i \in \boldsymbol{x}$, if it aligns with a word or several continuous words in $\boldsymbol{y}$, we add it to a candidate alignment set $\mathbf{A}$.To increase the scope of our modification, we also introduce add phrasal alignments to $\mathbf{A}$ through the following steps.
we first use Stanza~\footnote{https://stanfordnlp.github.io/stanza/} to find out all the phrases in $\boldsymbol{x}$ and $\boldsymbol{y}$, then take those that are covered by the word-to-word alignment as our segment-level alignments. 
\fi
If a longer segment overlaps with another shorter segment, we will only keep the longer segment % since substituting a word in a phrase might hurt the semantic meaning of the sentence
. To make the generation process more meaningful, for the first two types of segments, we limit the part of speech of the word to be noun, verb, adjective and adverb. Finally, we get a set of segment-level alignments $\mathbf{A}$ for $(\boldsymbol{x}, \boldsymbol{y})$.
%while removing stopwords and punctuations. 
%To avoid strange linguistic phenomenon during generation, we limit the part of speech of the extracted word to be noun, verb, adjective and adverb.

%we constrain that only segments in the source sentence $\boldsymbol{x}$ that have explicit alignments in $\boldsymbol{y}$ can be modified during our bilingual translation pair generation process. In this way, we can start from changing these aligned positions and make the best use of the rest parts of $\boldsymbol{y}$ when rephrasing $\boldsymbol{y'}$, which helps ensuring its quality.
\begin{table*}[tb]
  \renewcommand\arraystretch{1.1}
  \centering
  \setlength{\tabcolsep}{1.5mm}
  \small
  \begin{tabular}{p{1.7cm}p{13cm}}
    \toprule[1pt]
    \textbf{Method} & \textbf{Prompt} \\
    \midrule[0.5pt]
    \textbf{ChatGPT } & \texttt{"role": "system", "content": "You are a helpful assistant that translates English to Chinese.", "role": "user", "content": "[SRC]"}\\
    \textbf{ChatGPT Bi} & \texttt{"role": "system", "content": "You are a helpful assistant that translates English to Chinese.", "role": "user", "content": "You are given an English sentence and its Chinese translation. In each sentence, certain tokens have been masked with the '<mask>' token. Your task is to first fill in the masked tokens in the English sentence without modifying any of the unmasked tokens. Then, use the filled English sentence to fill in the masked tokens in its corresponding Chinese translation. If necessary, make modifications to the filled Chinese translation to ensure fluency while preserving the meaning. Finally, please output the filled English sentence and its filled Chinese translation in the format of 'Filled English:{} \textbackslash{}n Filled Chinese:{}'. \textbackslash{}n English Sentence: [MASKED ENGLISH]. \textbackslash{}n Chinese Translation: [MASKED CHINESE]"}\\
    \bottomrule[1pt]
  \end{tabular}
  \caption{Two prompts for querying the ChatGPT model.}
  \label{tab:prompts}
\end{table*}

\paragraph{Generating New Bilingual Translation Pairs}
\label{generating}
After obtaining segment-level alignments, we start to generate new bilingual translation pairs using the mask-then-infill strategy. Specifically, for each $(\boldsymbol{x}, \boldsymbol{y})$ pair along with its segment-level alignments, we randomly mask several aligned segments in $\mathbf{A}$ to create a masked pair $(\boldsymbol{\hat{x}}, \boldsymbol{\hat{y}})$, while making sure that the number of masked words in $\boldsymbol{\hat{x}}$ is less than $0.2 \times \text{len}(\boldsymbol{x})$. We repeat the above steps and construct at most 20 distinct masked pairs for each translation pair $(\boldsymbol{x}, \boldsymbol{y})$. %We do not mask the start of $\boldsymbol{x}$ for simplicity. 

Finally, we craft new bilingual translation pairs through filling in the masked pairs. Previous text infilling works can be mainly split into two categories: filling in a monolingual sentence~\cite{zhu2019text,donahue2020enabling} or a target sentence based on its corresponding source sentence~\cite{chen2021lexically,wang2022template, xiao2022bitiimt}. However, these techniques can not be directly adapted to our task since we need to fill in both $\boldsymbol{\hat{x}}$ and $\boldsymbol{\hat{y}}$. An intuitive way to complete this task is to first use a language model to fill in $\boldsymbol{\hat{x}}$ and obtain $\boldsymbol{x'}$, then fill in the target sentence $\boldsymbol{y'}$ with the second category of text infilling techniques. Yet these methods tend to fill in the translation of the filled source tokens, thus usually make the filled target sentence $\boldsymbol{y'}$ not fluent.


Recently, the large language model ChatGPT~\footnote{https://chat.openai.com/} designed by OpenAI has shown impressive performances on various NLP tasks including text generation and machine translation~\cite{qin2023chatgpt,jiao2023chatgpt,hendy2023good,peng2023towards} However, ChatGPT is still struggling with generating unbiased translations without hallucinations~\cite{hendy2023good,guerreiro2023hallucinations} when handling machine translation tasks. To tackle this issue and make the best use of the power of ChatGPT, we propose to incorporate the crafted masked pairs that contain semantic information of the original translation pairs to build prompts for generating bilingual translation pairs.
%build effective prompts for generating fluent and accurate bilingual translation pairs. 
Given a masked pair $(\boldsymbol{\hat{x}}, \boldsymbol{\hat{y}})$, we first instruct ChatGPT to fill in the masks in $\boldsymbol{\hat{x}}$, then fill in the masks in $\boldsymbol{\hat{x}}$ based on the filled source sentence. We also guide ChatGPT to paraphrase the filled sentences to ensure fluency. %In this way, we could fuse the information of the original translation pair are able to prompt ChatGPT to generate fluent and accurate translation pairs 
The prompt template is shown in the second row (\textbf{ChatGPT Bi}) of \tref{tab:prompts}. Once we obtain various bilingual translation pairs from ChatGPT, We filter out pairs that are the same as their original counterpart and keep the rest as the final translation pairs.

==> sections/quality.tex <==
\section{Intrinsic Evaluation}
\label{quality}

\subsection{Data}
We evaluate our proposed bilingual translation pair generation method using data extracted from the test set of the WMT21/22 En-Zh/Zh-En news translation task. We randomly sampled 200 generated pairs for evaluation.

\subsection{Evaluation Methods}
\label{evaluate method}
We perform automatic and manual evaluation to evaluate the quality of our bilingual translation pair generation method from three perspectives: source sentence fluency, target sentence fluency and translation adequacy.

\paragraph{Source Sentence Fluency} 
measures whether the filled source sentence $\boldsymbol{x'}$ is semantically meaningful and grammatically correct. For automatic evaluation, we calculate the perplexity score (\textbf{PPL}) of $\boldsymbol{x'}$ using the pre-trained GPT-2 language model~\cite{radford2019language}, where a lower score indicates higher fluency. As for human evaluation, we ask human annotators to score the fluency of the filled source sentence based on a three-point rating scale, in which 1/2/3 represents unsatisfied/fair/satisfied, respectively.

\paragraph{Target Sentence Fluency.} Similar to the source sentence fluency, it measures whether the filled target translation $\boldsymbol{y'}$ is semantically meaningful and grammatically correct, while not considering $\boldsymbol{x'}$. Likewise, we use perplexity as the automatic evaluation metric and adopt the same three-point scale to score each $\boldsymbol{y'}$ during human evaluation.

\paragraph{Translation Adequacy} captures whether $\boldsymbol{y'}$ has translated all the semantic information conveyed by $\boldsymbol{x'}$. Since we do not have a gold reference for $\boldsymbol{x'}$, we apply the reference-free version of the widely used metric COMET (\textit{wmt20-COMET-qe-da)}~\cite{rei-etal-2020-unbabels} that fuses direct assessments (DA), Multidimensional Quality Metrics error annotations, and sentence-level scores to automatically measure translation adequacy~\footnote{We do not use the latest wmt22-COMETkiwi-da model since it is currently unavailable.}, where a higher score indicates a more adequate translation. For human evaluation, we ask annotators to compare $\boldsymbol{x'}$ and $\boldsymbol{y'}$ word-by-word and give a score for $\boldsymbol{y'}$ following the same three-point scoring scale as source sentence fluency. 

For each of the human evaluation task, we invite three annotators who are proficient in both the source and the target language to rate the given text and they achieve a Krippendorff's alpha score~\cite{castro-2017-fast-krippendorff} of xx/xx/xx, respectively, indicating a high inter-agreement. For detailed instructions of our human evaluation, please refer to Appendix X.

\subsection{Baselines}
\label{quality baseline}
To illustrate the effectiveness of our proposed method, we compare it with two baselines:
\begin{itemize}
    \item \textbf{BART+BiTIMT.} This approach is a combination of two strong text infilling models. On the target side, we adopt the BiTIMT model~\cite{xiao2022bitiimt}, a strong method that infills tokens on top of the source sentence. To further enhance the fluency of the filled target sentence, we predict the whole target sentence $\boldsymbol{y'}$ instead of the filled tokens during the decoding process. For source sentence infilling, we apply the widely used BART model~\cite{lewis2019bart} whose pre-training task includes text infilling.
    \item \textbf{Ref.} Since we aim to construct high-quality translation pairs, we are interested about how well our crafted translation pair is comparing to manually created translation pairs. Specifically, we use the 200 original translation pairs that are used to construct the new translation pairs for comparison.
\end{itemize}

\begin{table}[tb]
  \renewcommand\arraystretch{1.1}
  \centering
  \setlength{\tabcolsep}{1mm}
  \small
  \begin{tabular}{lcccccc}
    \toprule[1pt]
    & \multicolumn{2}{|c|}{\textbf{Source}} & \multicolumn{2}{c|}{\textbf{Target}} & \multicolumn{2}{c|}{\textbf{Translation}} \\
    \midrule[0.5pt]
     \textbf{Method}& \textbf{PPL} & \textbf{H} & \textbf{PPL} & \textbf{H} & \textbf{COMET} &\textbf{H} \\
    \midrule[0.5pt] 
     \textbf{BART+BITIMT} & & 2.69& &2.57 & & 2.39\\
     \textbf{REF} &  &2.92 & &2.88 & &2.78 \\
     \textbf{Ours} &  & 2.92& & 2.84& & 2.80\\
    \bottomrule[1pt]
  \end{tabular}
  \caption{The quality of our method.\jw{In this section, the automatic evaluation can also be implemented on the 40000 dataset}}
  \label{tab:prompts}
\end{table}
\subsection{Results}





